Grounded Intuition of GPT-Vision's Abilities with Scientific Images

GPT-Vision has impressed us on a range of vision-language tasks, but it comes with the familiar new challenge: we have little idea of its capabilities and limitations. In our study, we formalize a process that many have instinctively been trying already to develop "grounded intuition" of this new model. Inspired by the recent movement away from benchmarking in favor of example-driven qualitative evaluation, we draw upon grounded theory and thematic analysis in social science and human-computer interaction to establish a rigorous framework for qualitative evaluation in natural language processing. We use our technique to examine alt text generation for scientific figures, finding that GPT-Vision is particularly sensitive to prompting, counterfactual text in images, and relative spatial relationships. Our method and analysis aim to help researchers ramp up their own grounded intuitions of new models while exposing how GPT-Vision can be applied to make information more accessible.

==> old/old_introduction.tex <==
\section{Introduction}
\subsection{Motivation}
The recent release of GPT-Vision \citep{openai_gptvision_2023} has ignited widespread fascination and inspiration for multimodal language models. One highlighted area of interest from the original paper is ``scientific proficiency.'' Scientific papers contain a wide variety of special content like graphs, diagrams, photos, computer code, and mathematical characters. Many of these elements are inaccessible to people with disabilities like vision or information processing disorders. Tools for generating alt text or explanations for these images---perhaps even adapted to each reader---can substantially increase accessibility while offering all readers opportunities to learn more deeply. Beyond reading, textual descriptions of images can allow users of audiobooks and screen readers to access visual content that has been out of reach for a long time. Preliminary exploration of GPT-Vision has shown great promise for all of these goals, but evaluating it can be a daunting task: generated text can run longer than a page and the possible configurations of images and prompts are endless. Just gaining initial familiarity with each new LLM can feel near impossible, let alone a decent grasp of its capabilities and limitations. In our work, we attempt to develop ``grounded intuition'' of GPT-Vision's abilities with scientific figures by leveraging qualitative analysis methods from social science and human-computer interaction research.

Prominent recent work studying LLMs have focused on qualitative, example-driven analysis, but this process can be time-consuming and laborious when generated text reaches a paragraph or even a page in length~\citep{bubeck_sparks-artificial-general_2023, yang_dawn-lmms-preliminary_2023}. The first major study to adopt this approach apologized for its methodology, acknowledging that it ``is somewhat subjective and informal, and that it may not satisfy the rigorous stands of scientific evaluation''~\citep{bubeck_sparks-artificial-general_2023}, but this method of qualitative analysis is remarkably comparable to well respected methods in social sciences and Human-Computer Interaction. Along with our analysis, we contribute a formalization of a qualitative analysis method for LLMs based on grounded theory~\citep{blandford_grounded-theory_2022}, which we have informally called the CREDA method.

Our analysis offers insight on GPT-Vision's \textit{behavior} with scientific images, which should not be conflated with a statistical understanding of how often it occurs or a scientific explanation of why. Even a suitable description of an image does not necessarily mean that GPT-Vision ``explained the image'' if the same information could have been hallucinated from its internal knowledge or training data. Much like the psychological origins of artificial intelligence, \textit{artificial behaviorism} cannot fully account for \textit{artificial cognition} or \textit{artificial neuroscience}. Further investigation on the ``cognitive'' processes of LLMs, like attention and memory, and the mathematical basis of neural networks is crucial for understanding LLMs holistically. To evaluate GPT-Vision for these goals, we conduct a deep, structured qualitative analysis of 23 scientific images including photos, diagrams, graphs, tables, mathematical text, computer code, and screen shots of full pages.

\subsection{Background}
\label{sec:bgrw}

Now that large language models are capable of producing such sophisticated output for a wide range of requests, ``evaluating generated text is now about as hard as generating it'' \citep{neubig_my-nlp-model_2023}. Recent work has warned us against relying on long-used automatic metrics for tasks like machine translation~\citep{fomicheva_taking-mt-evaluation_2019}, question answering~\citep{chen_evaluating-question-answering_2019}, and summarization~\citep{jain_multi-dimensional-evaluation-text_2023, goyal_news-summarization-evaluation_2023} because they may fail to accurately assess novel and abstractive text against a gold standard. Even reference-free metrics have been shown to underestimate the quality of generated text, perhaps because those metrics were trained or evaluated on the same reference-based benchmarks~\citep{goyal_news-summarization-evaluation_2023}. Automatic metrics have long been criticized for unreliably correlating with human judgment, even before the rise of LLMs~\citep{deutsch_statistical-analysis-summarization_2021, belz_comparing-automatic-human_2006}. Reference-free metrics are disproportionately weak at evaluating alt text for blind and low-vision readers~\citep{kreiss_context-matters-image_2022}. Some work has attempted to mitigate these challenges by using an intermediary LLM to evaluate generated text~\citep{liu_g-eval-nlg-evaluation_2023, ding_gpt3-data-annotator_2023a}, designing AI tools to aid data annotation~\citep{gao_collabcoder-gpt-powered-workflow_2023}, or improve metrics and datasets for new LLMs~\citep{jain_multi-dimensional-evaluation-text_2023, zhong_agieval-human-centric-benchmark_2023, sawada_arb-advanced-reasoning_2023}. We focus primarily on qualitative analysis.

Recent example-driven qualitative analyses of GPT-4 and GPT-Vision have already stepped toward robust qualitative analysis for modern LLMs~\citep{bubeck_sparks-artificial-general_2023, openai_gptvision_2023, yang_dawn-lmms-preliminary_2023}. While these studies tend to provide brief commentary on a large number of tasks and examples, we examine a small set of results more deeply through a method based on grounded theory~\citep{blandford_grounded-theory_2022} and thematic analysis~\citep{blandford_thematic-analysis_2022}, which are frequently used in human-computer interaction research. Grounded theory is a data-driven or ``bottom-up'' perspective on data collection and analysis. In grounded theory, patterns and conclusions ``emerge'' from the data, much like an inductive analysis~\citep{bingham_qualitative-analysis-deductive_2023}. Grounded theory instructs analysts to make meaning solely from the data to avoid bias from preconceived notions or existing theories. It includes a method called theoretical sampling, which is based on the idea that we can carefully select data that contains characteristics we care about as opposed to sampling at random or gathering a large dataset~\cite{blandford_sampling_2022}. Theoretical sampling also allows data to be gathered iteratively to address findings as they arise throughout the analysis until we hit ``theoretical saturation'': a subjective yet evidence-based instinct that further data collection and analysis will not reveal any more major insights.

Thematic analysis is a flexible framework through which grounded theory can be applied. First, ``themes'' are gathered from the data, refined, and then applied to the entire dataset to reveal patterns within it. When adopted formally, thematic analysis is a rigorous process that can involve evaluating inter-annotator agreement and setting up infrastructure to protect reliability in qualitative research~\citep{mcdonald_reliability-inter-rater-reliability_2019}. It has been used regularly in well reputed HCI studies like supporting healthcare~\citep{bowman_using-thematic-analysis_2023}, analyzing social media posts~\citep{gauthier_will-not-drink_2022}, and conducting literature reviews~\citep{cooper_systematic-review-thematic_2022}. Brand-new work to be published in the Findings of EMNLP 2023 even proposes an LLM-in-the-loop collaboration framework to assist with thematic analysis~\citep{dai_llm-in-the-loop-leveraging-large_2023}. Our work adapts thematic analysis and grounded theory specifically for evaluating LLMs in NLP research.

Our analysis focuses on GPT-Vision's ability to describe scientific images. Past work on describing images has included automatic image captioning~\citep{tang_vistext_2023, hsu_scicap-generating-captions_2021, spreafico_neural-data-driven-captioning_2020, guinness_caption-crawler-enabling_2018} and alt text generation~\citep{wu_automatic-alt-text-computer-generated_2017, salisbury_scalable-social-alt_2017, williams_quality-alt-text_2022, chintalapati_dataset-alt-texts_2022}. Alt text is a written version of an image that appears in place of it~\citep{vleguru_alt-text-video_2022}. Although alt text is typically associated with screen readers and vision loss, it can also help users with information processing disorders, like issues with visual sequencing, long- or short-term visual memory, visual-spatial understanding, letter or symbol reversal, or color blindness~\citep{mccall_rethinking-alt-text_2022}. Alt text can even help in purely situational circumstances like broken image links or loading issues due to expensive data roaming or weak internet connectivity, which may disproportionately affect individuals with lower incomes~\citep{vleguru_alt-text-video_2022}. Beyond reading online documents, alt text and curated image descriptions can allow audio books and screen readers to ``read aloud'' visual content, giving all of us even more access to news articles, textbooks, blog posts, scientific papers, and other mixed-media texts. These image descriptions, however, need to be generated carefully and, most likely, adaptively.  Alt text by definition depends on the audience, content, and situation, so one approach will not work for all images or people~\citep{w3_images-tutorial_2022}. This claim was validated in practice by a user study~\citep{stangl_going-beyond-one-size_2021}. Blind and sighted readers diverge~\citep{lundgard_accessible-visualization-natural_2021}. Even placement of text has an impact~\citep{stokes_striking-balance-reader_2022}.


Part of this analysis is ``objective,'' such as detecting objects, transcribing labels, and identifying spatial positions, but many aspects are inherently human-centered. What is the ``correct'' interpretation of a graph or the ``main idea'' of a diagram? What is an ``appropriate'' description---not too long, not too short, not too detailed, not too vague? Now that LLMs are so powerful and widely used, we need to address what we as users want from the model beyond just the facts, which we can start to investigate through the human-centered design framework~\citep{norman_design-everyday-things_2013}. We should also acknowledge that different users have different needs, which are often affected by their differing abilities. The same ability can vary in duration and context---consider a user who can needs to have a book read aloud because they are blind, are in a dark room, or had their pupils dilated---as suggested by the ability-based design framework~\citep{wobbrock_ability-based-design-concept_2011}. Together, ability-based human-centered design can help us build inclusive tools for everyone~\citep{Hwang_Build_Your_Own_2023}. 

\subsection{Contributions}
In this paper, we contribute:

\begin{itemize}
    \item Deep, grounded insights on GPT-Vision describing scientific images
    \item A qualitative analysis framework based on grounded theory and thematic analysis for evaluating LLMs
    \item The images we used and the text we generated for future work and reproducibility
\end{itemize}

Part of our goal was to formalize a process that people have already naturally taken to evaluate LLMs: trying a selection of images and prompts, skimming through generated text, and noticing patterns until we are satisfied with our ``intuition.'' Our method provides an organized, systematic framework for intentionally developing this intuition grounded in concrete data. A practical guide on our method and theoretical background will be released soon.

==> sections/5_figures.tex <==
\section{Figures}
\label{sec:figures}

Here we focus on figures, which we defined as standalone elements with captions that could be placed arbitrarily on the page. We studied four major categories of figures: photos (P1--2 [\ref{app:p1}, \ref{app:p2}]), diagrams [D1--3 (\ref{app:d1}, \ref{app:d2}, \ref{app:d3})], graphs (G1--4 (\ref{app:g1}, \ref{app:g2}, \ref{app:g3}, \ref{app:g4})), and tables (T1, \ref{app:t1}; T2, \ref{app:t2}; T3, \ref{app:t3}).
% (T--3 (\ref{app:t1}, \ref{app:t2}, \ref{app:t3})).
To discuss these figure types, we chose one representative image per type to discuss in more detail. The complete set of inputs and outputs can be found TODO.

\subsection{Photos}

\begin{quote}
    kitchen photo here
\end{quote}

%%% moved to findings %%%
P2 (\ref{app:p2}) is a photo of a female study participant cooking a dish in a kitchen with the guidance of a voice assistant. The voice assistant, a blue spherical Alexa Echo Dot, is displayed on the right side of the image with a circle around it.

\paragraph{Incorporation and lack of context} Although the type of device circled in image is not immediately clear, the caption that was given as additional context stated that ``[participants] followed recipes of their own choice with the help of Amazon Alexa (Echo Dot, dircled on the right)'' \citep{hwang_rewriting_2023}. GPT-Vision incorporated this information well for the ``desc'' prompt,

\begin{quote}
    What stands out is an Amazon Alexa Echo Dot, which is circled for emphasis. It is placed to the far right on the countertop near some other kitchen tools. (P2 desc, \ref{app:p2})
\end{quote}

\noindent but not for the ``alt'' prompt.

\begin{quote}
    There is a small circular clock with a white frame hanging on the wall, indicated by a circle. (P2 alt, \ref{app:p2})
\end{quote}

In most cases, information from the context did not appear in the generated passages. This suggests that GPT-Vision ``ignored'' it, but we cannot know for sure based on our behavioral evaluation. We do, however, have evidence that GPT-Vision has the capacity to leverage text and image inputs at the same time.

D3 alt (\ref{app:d3}), P1 desc (\ref{app:p1}), P2 desc (\ref{app:p2}), and G2 alt (\ref{app:g2}) show similar examples of incorporating context. D3 alt and desc (\ref{app:d3}), T1 alt and desc (\ref{app:t1}), P2 alt (\ref{app:p2}), T2 alt (\ref{app:t2}), T3 alt and desc (\ref{app:t3}), D1 alt and desc (\ref{app:d1}), G1 alt and desc (\ref{app:g1}), G2 alt and desc (\ref{app:g2}), and G4 alt and desc (\ref{app:g4}) contain similar behavior of lacking context.
%%% moved to findings %%%

\paragraph{Interpretations and inferences} When describing a photo, GPT-Vision usually tended toward literal interpretation for the ``alt'' prompt like ``The kitchen features white tiles... and various cooking utensils and ingredients'' (P2 alt, \ref{app:p2}). For the ``desc'' prompt, GPT-Vision frequently expanded on the visual details to varying degrees of reliability.

In one case, GPT-Vision states that 

\begin{quote}
    Her [the participant's] face is not visible as it's blurred for privacy reasons. (P2 desc, \ref{app:p2})
\end{quote}

\noindent GPT-Vision infers that she/her/hers pronouns should be used with this participant, which is true for this individual, but we may want to be more careful assuming genders based solely on physical appearance.

Furthermore, GPT-Vision's assertion that the participant's face is blurred for privacy reasons, while probable, is not grounded in the input---the image and context never say why the face has been blurred. The assertion turns out to be correct, so we could say that GPT-Vision ``inferred'' it, but if it had been wrong then it would be classified as a ``hallucination.'' 

This is particularly important when GPT-Vision is wrong. When describing the pictured Amazon Alexa Echo Dot, it says

\begin{quote}
    The Echo Dot is of a prior generation, as it is not spherical but rather has a horizontal cylindrical shape. (P2 desc, \ref{app:p2})
\end{quote}

\noindent The Echo Dot in the photo is a fourth-generation model \citep{amazon_dot-4_2020}, which was two years prior to the current fifth-generation model \citep{amazon_dot-5_2022}. Both of models, however, share the same \textit{spherical} shape. Neither are ``cylindrical,'' although past generations of the Echo Dot could be considered a ``flat cylinder'' while past generations of the original Echo could be considered a ``tall cylinder'' \citep{amazoncustomerservice_which-echo-device_2022}. The meaning of ``horizontal cylinder'' is unclear, but it could be a cylinder that is lying on its curved side rather that one of its flat sides. None of the Alexa devices seem to have this shape \citep{amazoncustomerservice_which-echo-device_2022}. See figure TODO.

\begin{quote}
    figure of echo shapes here
\end{quote}

Accuracy aside, end-users may appreciate knowing when LLMs are interpreting or reiterating so they can judge for themselves how much to trust the generated passage.

\paragraph{Object recognition} Beyond the intricacies of incorporating context and mitigating interpretation, GPT-Vision consistently recognized real-life objects in photos quite well. It recognized many kitchen implements in P2 (\ref{app:p2}) (but hallucinated a kitchen sink in both generated passages), aptly described the stove and which burner the participant was using (desc), and accurately described the spatial positions of various elements in the image (desc). P1 alt and desc (\ref{app:p1}) contain some attempts at object recognition as well.

\subsection{Diagrams}

\begin{quote}
    kani diagram here
\end{quote}

D1 is the diagram from the first page of \citet{zhu_kani_2023}, providing an overview of a new framework for building chat-based LLM applications called Kani. The main part of the diagram is a square box representing a Kani application, which is labeled with the word ``Kani'' and the crab logo. The Kani box contains three boxes representing ``Chat History,'' ``Function Context,'' and ``Engine.'' Outside the Kani box, an avatar of a human is asking, ``What's the weather like in Tokyo?'' in a speech bubble. Kani replies in another speech bubble, ``It's 22 degrees Celsius and sunny in Tokyo right now.''

\paragraph{Visual-spatial details} As usual, GPT-Vision relies heavily on visual and literal features when describing diagrams. The spatial details are usually correct, like stating that the user interacting with Kani is on the left, Kani is on the right, and the avatar representing the user has a laptop (alt and desc). It does get a few details wrong, however: saying that the user avatar is sitting at a desk (desc) and hallucinating an ``emoji of a face wearing sunglasses,'' for example (desc).

%%% moved to findings %%%
\paragraph{Struggles with boundaries} GPT-Vision has adeptly described individual elements in many generated passages, but it struggled a lot with overlapping elements in D1. The Kani box contains the label ``Kani'' with the crab logo followed by three boxes stacked on top of each other: green ``Chat History'' on top of pink ``Function Context'' on top of yellow ``Engine.'' However, in GPT-Vision's words,

\begin{quote}
    The top section of this [the Kani box] shows a chat history window. The window has the name `Kani' at the top and next to the name there is a red crab icon... Just below the chat history window, there is a section called `Function Context.' ... It's in a box with rounded edges and a light yellow background. (D1 desc, \ref{app:d1})
\end{quote}

\noindent GPT-Vision blurs a few details here. The label `Kani' with the crab is at the top of the diagram but \textit{outside} the Chat History box. The Function Context box is directly below Chat History, but it is actually pink. The Engine box, which is under Function Context, is yellow. This mix-up between nearby visual elements also occurs in P1 desc (\ref{app:p1}). The diagram according to GPT-Vision would like more like Figure TODO.
%%% moved to findings %%%

\paragraph{Contextual errors}
GPT-Vision misrepresented Kani as a chatbot rather than an LLM framework---it is a programming tool rather than the tool itself \citep{zhu_kani_2023}. This information was included in the caption (``Kani is a lightweight and flexible framework...'') and reference paragraph (``...we present Kani: a lightweight, flexible, and model-agnostic framework for developing LM applications.'') provided with the the image, but the information did not seem to ``transfer'' over to the output.

\paragraph{Interpretation} GPT-Vision makes a few good interpretations when describing D1, including that the diagram represents a conversation between a human and a computer (alt and desc). Its most impressive interpretation was of the Chat History section, which represents turns in the conversation has lines rather than actual text:

\begin{quote}
    Within this chat history window, there are several obscured chat bubbles... There aren't any explicit words or sentences visible inside this chat history window; the contents are blurred lines meant to represent text. (D1 desc, \ref{app:d1})
\end{quote}

\noindent Besides the overloaded meaning of ``explicit words or sentences,'' GPT-Vision described the main idea of this part of the diagram very well.

Not all of its interpretations were so good, however. It described the content of the Function Context as

\begin{quote}
    The code sample is not complete; it's meant to suggest that there is some programming involved in fetching the weather data. (D1 desc, \ref{app:d1})
\end{quote}

\noindent which is not completely accurate. The Function Context section contains function headers 

\begin{center}
    \texttt{def get\_weather(location: str)} and \texttt{def fahren\_to\_celsius(deg: int)}
\end{center}

\noindent to indicate that similar headers can be passed to Kani to allow the underlying language model to call functions. GPT-Vision's claim is not necessarily incorrect and this information is not included in the context it received, but controlling interpretation is an important part of preventing misinformation.

%%% moved to findings %%%
\paragraph{(Lack of) logo recognition} GPT-Vision also failed to recognize the three logos displayed in the ``Engine'' section at the bottom of D1. These logos were supposed to represent the language models that Kani supports:

\begin{enumerate}
    \item OpenAI (a circular logo resembling three intertwined chain links) \citep{openai_openai_2023},
    \item Hugging Face (a yellow emoji-like happy face with open hands) \citep{huggingface_hugging-face_2023},
    \item LLaMA (not an official logo, a brown cartoon llama with the Meta logo) \citep{touvron_llama-open-foundation_2023},
    \item Vicuna (head of a cartoon vicuna, which has a tall neck and pointy ears) \citep{thevicunateam_vicuna-open-source-chatbot_2023}.
\end{enumerate}

\noindent which GPT-Vision described in the desc passage as

\begin{enumerate}
    \item ``a caduceus [two serpents twisted on a winged staff, often associated with medicine] with only one snake'' \citep{wikipedia_caduceus_2023},
    \item ``a yellow smiley face,''
    \item ``a flamingo,'' and
    \item ``a letter `Y' with what looks like animal ears on top.''
\end{enumerate}

Besides mistaking the llama for a flamingo, GPT-Vision's descriptions of the engine icons are not far off, but not recognizing the logos themselves obscured the point of this part of the diagram. 
%%% moved to findings %%%

\subsection{Graphs}

\begin{quote}
    TODO figure
\end{quote}

This section discusses the three types of graphs we investigated in this study: bar charts (G1, \ref{app:g1}), line graphs (G3, \ref{app:g3}; G4, \ref{app:g4}), and pie charts (G2, \ref{app:g2}) (see Figure TODO or Appendix Section \ref{app:data}). 
% G1 (\ref{app:g1}), a bar chart, contains three subplots each representing two categories and four series of data (two groups of four bars per subplot) with error bars. G2 (\ref{app:g2}) is a three-by-three grid of nine pie charts showing the proportions of nine categories. G3 (\ref{app:g3}) and G4 (\ref{app:g4}) are both line graphs, but G3 shows a simpler plot of three lines overlaid by two benchmark lines. G4 is more complex: it shows three groups of two lines, solid and dashed, with additional information in annotations.

\paragraph{Misreading bar charts}
GPT-Vision consistently misconstrued the numeric values of G1 (\ref{app:g1}), a bar chart with three subplots. G1 shows the average number of all sentences with named entities and sentences with only novel named entities from 0.0 to 3.0 in increments of 0.5. Horizontal grid lines indicate each increment. These sentences belong to one of four groups, so each subplot displays two groups of four bars.

In the subplot representing the stories domain, GPT-Vision states that

\begin{itemize}
    \item ``human-written'' named entity sentences occurred ``just over 1.0'' times (actually below 0.5),
    \item ``machine-generated'' sentences occurred ``approximately 1.5'' times (actually a little above 0.5),
    \item sentences that were ``never selected by player'' occurred ``close to 1.2'' times (actually just above 0.5), and
    \item sentences that were ``selected by $\geq$ 1 players'' occurred ``around 1.3 times'' (actually about halfway between 0.5 and 1.0). (G1 desc, \ref{app:g1})
\end{itemize}

Each of these estimates are drastically different from their real values, suggesting that GPT-Vision struggles to ``read'' axes. It showed the same behavior on line graphs as well (G3, \ref{g3}; G4, \ref{app:g4}). It may struggle because error bars are overlapping data bars which are overlapping axis grid lines, similar to how GPT-Vision poorly described some of the overlapping elements in D1 (see Section TODO). These estimates were still clearly when taking error bars into account based on where the error bars cross the grid lines.

GPT-Vision performed even worse when trying to describe a more general trend:

\begin{quote}
    Novel named entities are lower with averages between 0.6 and 0.9. (G1 desc, \ref{app:g1})
\end{quote}

\noindent The bars in the ``novel named entity'' group are too similar to say definitively that they are lower than the bars in the ``named entities'' group. More importantly, these bars range from about 0.25 to about 0.75. Three out of four of the bars barely reach the lower bound of this range. GPT-Vision performed similarly on the other two subplots in this figure.

\paragraph{Misinterpreting line graphs}

GPT-Vision also struggled with line graphs, like G3 (\ref{app:g3}) and G4 (\ref{app:g4}). Both were sourced from \citet{brown_gpt3-few-shot_2020}, which introduced GPT-3. G3 shows the accuracy of zero-shot, one-shot, and few-shot prompting as GPT-3 increases from 0.1 to 175 billion parameters.

G4 is more complex. It shows the accuracy of 1.3 billion--, 13 billion--, and 175 billion--parameters as the number of in-context examples grows from 0 to 32. Each model size is represented by two lines: a solid line for a ``Natural Language Prompt'' and a dashed line for ``No Prompt.'' The graph contains free-floating labels for prompt style and model size as opposed to a legend, like in G3.

GPT-Vision described the x- and y-axes of each line graph moderately well, with one idiosyncrasy. The y-axis in G4 (\ref{app:g4}) is linear, going from 0 to 70 in increments of 10. However, 70---the top of grid---is not labeled. The labels stop at 60, with a blank space where ``70'' would have been. GPT-Vision does not make this distinction:

\begin{quote}
    The y-axis, or vertical axis, is labeled ``Accuracy (\%)'' and has a linear scale ranging from 0 to 60. (G4 desc, \ref{app:g4})
\end{quote}

\noindent This inaccuracy is particularly striking because the data in the graph goes beyond 60\%, which could confuse the reader. GPT-Vision exhibited similar behavior across graphs, including the bar graphs in G1 (\ref{app:g1}). It showed signs of bias toward text in the image several times throughout the study, including labels of photos (see Section TODO) and captions of figures (see Section TODO).

GPT-Vision made a subtler text-based error when describing the x-axis in G4 (\ref{app:g4}):

\begin{quote}
    The x-axis, or horizontal axis... has a logarithmic scale, starting at 10\^{}0 and increasing to 10\^{}1. (G4 desc, \ref{app:g4})
\end{quote}

\noindent The x-axis is labeled with ``$0$,'' ``$10^0$,'' and ``$10^1$,'' reminiscent of a logarithmic scale, but ``$10^1$'' is further away from ``$10^0$'' than ``$10^0$'' is from ``$0$.'' These values would be equally spaced in a true logarithmic scale. Combined with its apparent trouble to estimating values on an axis (see ``Misreading bar graphs''), distinguishing overlapping elements (see ``Struggles with boundaries'' in Section TODO), and predicting bounding boxes for object detection \citep{openai_gptvision_2023}, GPT-Vision may have a problem with perceiving distances.

GPT-Vision also imprecisely represented data trends in both line graphs. G3 (\ref{app:g3}), for example, displays three solid lines with circle markers for ``Zero-Shot'' (blue), ``One-Shot'' (green), and ``Few-Shot (K=15)'' (orange) prompting. It described the lines qualitatively with some clarity:

\begin{quote}
    The third line, depicted in blue and labeled ``Zero-Shot'', appears to be an upward leaning curve... The fourth line, represented in green and labeled ``One-Shot'', is similar to the third but starts at a slightly higher accuracy... Lastly, an orange line labeled ``Few-Shot (K=15)''... increases quite sharply... (G3 desc, \ref{app:g3})
\end{quote}

The Few-Shot (K=15) line does increase more sharply relative to the other two, but perhaps not in the absolute sense. It rises at a roughly 45$^\circ$ angle, which was ambiguously steep in our view. The Zero-Shot and One-Shot curves do look similar to each other, starting low and rising gently. The One-Shot line, however, starts at \textit{substantially lower} accuracy (about 20\%) than Zero-Shot (about 40\%).

GPT-Vision also imprecisely estimated the starting and ending values of each curve: it noted Zero-Shot as ranging from 30\% to 60\% (closer to 40\%--75\%), One-Shot from 40\% to 70\% (closer to 20\%--70\%), and Few-Shot (K=15) from 35\% to 90\% (closer to 20\%--85\%). It stated that Few-Shot (K=15) ``surpass[ed] the One-Shot accuracy at around 2.6 billion parameters,'' which is inaccurate as well---Few-Shot surpassed One-Shot much earlier, between 0.4 and 0.8 billion parameters.

Similar behavior occurred in both generated passages for G4 \ref{app:g4} as well.


%%% moved to findings %%%
\paragraph{Miscoloring pie charts}
% \paragraph{Mistaking colors in pie charts}

Unlike the bar and line graphs, GPT-Vision articulated the values of each slice of the pies in G2 (\ref{app:g2}). The catch: the values were labeled in G2 but not in the others. GPT-Vision properly transcribed text from images many times, but it mostly failed to estimate the magnitude of visual elements from size alone. GPT-Vision's greatest challenge with the pie charts was its apparent inability to recognize colors, as mentioned in \citet{openai_gptvision_2023}.

G2 (\ref{app:g2}) shows color mappings for nine error categories in a legend: 

\begin{quote}
    (1) ``grammar,'' (2) ``repetition,'' (3) ``irrelevant,'' (4) ``contradicts\_sentence,'' (5) ``contradicts\_knowledge,'' (6) ``common\_sense,'' (7) ``coreference,'' (8) ``generic,'' and (9) ``other.'' 
\end{quote}

\noindent GPT-Vision reported a shorter, slightly different list of categories (\textbf{emphasis} ours):

\begin{quote}
    (1) ``grammar errors,'' (2) ``repetition\textbf{s},'' (3) ``irrelevan\textbf{ce},'' (4+5) ``contradictions with sentence context or knowledge,'' (6+) ``commonsense \textbf{and coherence} errors,'' (7) ``coreference errors,'' and (8) ``other errors.'' (G2 desc, \ref{app:g2})
\end{quote}

It mislabeled most of the colors (see Table TODO). It mistook green for blue, orange for green, pink for yellow, light green for light purple, yellow for orange, and tan for red (G2 desc, \ref{app:g2}). Some of mistaken pairs were similar to each other, but several of them were completely different. GPT-Vision displayed similar behavior with the legend in G1 (\ref{app:g1}) as well, suggesting that color recognition is a serious weakness for it.
%%% moved to findings %%%

\subsection{Tables}

\paragraph{Presenting rows in context}

\paragraph{Reciting rows and columns, with counting errors}

\paragraph{Tripping over multirows and multicolumns}

\paragraph{Missing cells}

\paragraph{Interpreting table trends}

==> sections/6_full-pages.tex <==
\section{Full Pages}
\label{sec:full-pages}

\subsection{Summarization}
\subsection{Lossy Expansion}

==> sections/7_lang-comp.tex <==
\section{Language and Composition}
\label{sec:lang-comp}

In this section, we discuss GPT-Vision's portrayal of special text (code and math) and writing style (persona and writing mechanics).

%%% moved to findings %%%
\subsection{Code}
% \label{sec:code}

Several input images included some form of code:

\begin{itemize}
    \item C1 (pseudocode algorithm shown in Appendix Section \ref{app:c1})
    \item C2 (Haskell proof shown in Appendix Section \ref{app:c2})
    \item C3 (Python class definition and instance methods shown in Appendix Section \ref{app:c3})
    \item F5 (Screenshot of full page with Haskell code snippets shown in Appendix Section \ref{app:f5})
    \item D1 (diagram of Kani, a framework for LLMs shown in Appendix Section \ref{app:d1})
\end{itemize}

In general, GPT-Vision's descriptions of code were accurate and high-level. It correctly indicates that C3 ``contains a screenshot of Python code which defines a class named `LlamaEngine' that inherits from `HuggingEngine'{}'' (C3 alt, \ref{app:c3}) and that the class ``has three methods: `\_\_init\_\_', `build\_prompt', and `message\_len'{}'' (C3 alt, \ref{app:c3}). It even elaborates on the methods, such as correctly stating that ``the `build\_prompt' is meant for building and tokenizing a prompt from a user-assistant conversation, using incoming messages and functions. It accepts messages and functions as parameters and appends tokens to build a prompt'{}''  (C3 alt, \ref{app:c3}). When queried with the ``desc'' prompt, GPT-Vision provides even more specific details: ``the \`{}build\_prompt\`{} method... accepts two parameters: `self', which is standard for class methods, and 'messages', which is expected to be a list of ChatMessage'' (C3 desc, \ref{app:c3}). These details, while correct, may not be the most helpful overview of piece of sophisticated code that incorporates special tokens depending on the chat role and specifies particular types of expected inputs through Python type annotations. GPT-Vision even misprints one of the types as ``SomeFunction'' rather than ``AIFunction'' (C3 desc, \ref{app:c3}). With further human-centered studies on user needs, GPT-Vision shows promising potential for Python code explanation.

GPT-Vision also ``translates'' pseudocode to natural language quite well, besides some errors in reproducing mathematical text (see Section~\ref{sec:math} for more details). C1 contains an if statement in two nested for loops to demonstrate an dynamic matching algorithm. Instead of reproducing the pseudocode verbatim, it describes it more generally:

\begin{quote}
    The algorithm starts by calculating the solution to `LP-UB' and stores it in `$\alpha xy$'. Then, for each agent `i' arriving at time `t' of a certain type `y', and for each type `x' in a random order, it check if there's at least one unmatched agent `j' of type `x'. If so, agent `i' is matched with `j' with a calculated probability dependent on `$\gamma$' and `$\alpha xy$'. The algorithm terminates after processing all agents. (C1 alt, \ref{app:c1})
\end{quote}

\noindent When responding to the ``desc'' prompt, it breaks the pseudocode down into four steps:

\begin{enumerate}
    \item First, it calculates ``(a\_xy)''...
    \item The algorithm then enters a loop where for each agent ``i'' ..., it further loops through each type ``x''...
    \item Inside this nested loop, there is a conditional statement...
    \item If this condition is true, the algorithm matches agent ``i'' and ``j''... (C1 desc, \ref{app:c1})
\end{enumerate}

Descriptions of Haskell, however, tend to be much more superficial, like stating that C2 starts with ``the definition for a data type called \`{}Freer\`{}, followed by definitions for \`{}{}Return\`{}{} and \`{}{}Bind\`{}{}'' (desc, \ref{app:c2}) or ``[the] type alias \`{}Reflective\`{} [is] defined as \`{}Freer (R b)\`{}'' (alt, \ref{app:c2}). The difference between GPT-Vision's behavior with Python and Haskell may suggest that it is ``more familiar'' with the former.

Beyond code content, GPT-Vision displayed inconsistent behavior for code formatting. It used single quotes (`...'), double quotes (``...''), and backticks (\`{}...\`{}) to denote words directly reproduced from the image, sometimes mixing or even omitting the punctuation in the same passage: ``The \`{}build\_prompt\`{} method... accepts two parameters: `self'... and `messages', which is expected to be a list of ChatMessage'' (C3 desc, \ref{app:c3}). Code formatting style has direct implications for end-users reading textual descriptions. The differing formatting to represent the same concept may be confusing. The backticks are consistent with Markdown formatting for code, but the viewing system may not render them correctly. Finally, these punctuation marks may not translate well to audio books or screen readers. Depending on the user and situation, code needs to signified differently.
%%% moved to findings %%%

\subsection{Math}
\label{sec:math}

A few images displayed a fair range of mathematical text:

\begin{itemize}
    \item M1 (equations and explanation for a new language model architecture shown in Appendix Section \ref{app:m1})
    \item M2 (mathematical proof of a theorem in algorithmic theory shown in Appendix Section \ref{app:m2})
    \item C1 (pseudocode algorithm shown in Appendix Section \ref{app:c1})
    \item T3 (table of model training schemes depicted as exponentiated numbers shown in Appendix Section \ref{app:t3})
\end{itemize}

GPT-Vision produced numerous errors in reproducing mathematical text, from misprinting ``$1^5$'' as ``1\^{}5\^{}2'' (T3 desc, \ref{app:t3}) to misrepresenting ``$\left(\alpha - \frac{(1 - \alpha) 2mw(\left\lceil m \right\rceil) }{k-1} \right)$'' as ``$(\alpha - 1 / (2k - 2))$'' (C1 alt, \ref{app:c1}). These errors can have drastic consequences if they are not corrected or verified. GPT-Vision appears to reproduce mathematical text inconsistently in \LaTeX-style syntax or special characters. Some instances are as minute as reproducing the Greek letter alpha as ``$\alpha$'' in C1 alt (\ref{app:c1}) or (incorrectly) ``a'' in C1 desc (\ref{app:c1}).

Besides the downstream challenge that the end-user's system may not render \LaTeX, many of the \LaTeX-style reproductions are wrong. In the previously mentioned case, even if the end-user's system were compatible with \LaTeX, ``1\^{}5\^{}2'' would be return a compilation error. GPT-Vision sometimes omitted subscripts or misprinted them (which could be attributed to low resolution), but it \textit{always} represented multi-character subscripts incorrectly except for once. For example, GPT-Vision reproduced ``$\alpha_{xy}$'' from C1 as ``a\_xy'' (alt, \ref{app:c1})---which would be rendered as $a_xy$---and ``$\alpha$xy'' (desc, \ref{app:c1})---which would be rendered as $\alpha xy$. Perhaps fortunately, these types of errors were internally consistent within each passage.

The one multi-character subscript GPT-Vision reproduced correctly was from this equation: 

\begin{equation*}
    p(y_i | y1, ..., y_{i-1}, x) = g(y_{i-1}, s_i, c_i),
\end{equation*}

\noindent which it wrote as

\begin{center}
    p(y\_i$|$y\_1, ..., y\_\{i-1\}, x) = g(y\_\{i-1\}, s\_i, c\_i) (M1 desc, \ref{app:m1}).
\end{center}

\noindent Given the frequency of its \LaTeX \ errors and the ubiquity of this expression as a conditional probability for a recurrent neural network, we should avoid assuming that GPT-Vision ``understood'' how to print it correctly. GPT-Vision may actually need to be trained specifically for \LaTeX as a programming language, similar to Python or Haskell (see Section \ref{sec:code}). Descriptions of mathematical text could go even further by describing it in natural language, as GPT-Vision successfully did with the pseudocode algorithm in C1 (\ref{app:c1}, see Section \ref{sec:code}), especially for audio books and screen readers.



\subsection{Persona}
\subsection{Writing Mechanics}
\label{sec:writing-mech}
